Learning HMMs with Nonparametric Emissions via Spectral Decompositions of Continuous Matrices

Recently, there has been a surge of interest in using spectral methods for estimating latent variable models. However, it is usually assumed that the distribution of the observations conditioned on the latent variables is either discrete or belongs to a parametric family. In this paper, we study the estimation of an $m$-state hidden Markov model (HMM) with only smoothness assumptions, such as H\"olderian conditions, on the emission densities. By leveraging some recent advances in continuous linear algebra and numerical analysis, we develop a computationally efficient spectral algorithm for learning nonparametric HMMs. Our technique is based on computing an SVD on nonparametric estimates of density functions by viewing them as \emph{continuous matrices}. We derive sample complexity bounds via concentration results for nonparametric density estimation and novel perturbation theory results for continuous matrices. We implement our method using Chebyshev polynomial approximations. Our method is competitive with other baselines on synthetic and real problems and is also very computationally efficient.

==> sections/implementation.tex <==
% !TEX root = ../paper.tex

\section{Implementation}
\label{sec:implementation}

In order to make the described algorithm practical, it should have an efficient and stable implementation.
The main questions is how to represent and compute with 1-, 2-, and 3-dimensional functions?
It turns out that this can be achieved by using Chebyshev polynomial approximations to continuous functions on compact domains.
Chebyshev polynomials can be defined recurrently as follows:
\begin{eqnarray}
    T_0(x) & = & 1,\\
    T_1(x) & = & x,\\
    T_{n+1}(x) & = & 2 x T_{n}(x) - T_{n-1}(x).
\end{eqnarray}
Any $L^2$ function can be approximated by Chebyshev series that converges absolutely and uniformly.
This powerful property allows to represent continuous 1-, 2-, and 3-dimensional functions up to a machine precision in a very efficient manner\footnote{Omitting the details on the iterative numerical procedures used to approximate any given function with the corresponding polynomial expansion, we should mention that in the 2- and 3-dimensional case, the functions are additionally represented with polynomials of low rank.}~\cite{trefethen2015computing}.
Moreover, thanks to analytical polynomial representation, many operations on these functions, such as integration and singular value decompositions, can be performed also efficiently.

Chebyshev polynomials are fundamental to make our proposed spectral learning algorithm computable.
Our implementations makes use of the \texttt{chebfun} library~\cite{driscoll2014chebfun} that implements all the standard algebraic operations for continuous functions.
All the functions in our algorithm, such as $\hat P_{1}$, $\hat P_{21}$, $\hat P_{321}$, are represented as \texttt{chebfun} objects for which the algebraic operations are overloaded.
This allows to execute SVD on C-matrices, perform pseudo-inverses, and convolutions in literally constant time.
Given a fixed approximation accuracy, converting KDE estimates, $\hat P_{1}$, $\hat P_{21}$, $\hat P_{321}$, into \texttt{chebfun} objects takes time linear in the number of training samples.


==> sections/obshmm.tex <==
% !TEX root = ../paper.tex

\section{Observable Representation for Nonparametric HMMs}

An HMM characterizes a probability distribution over a sequence of hidden
states $\{\hht\}_{t\geq 0}$ and observations $\{\xt\}_{t\geq 0}$. We consider a
model with $m$ possible hidden states, i.e., $\hht \in [m] =
\{1,\dots,m\}$, and observation in some bounded continuous domain $\Xcal$.
W.l.o.g., we take $\Xcal=[0,1]$ (high dimensional case is discussed in
Section~\ref{sec:conclusion}). $T\in\RR^{m\times m}$ denotes the
transition matrix where $T(i,j) = \PP(\hhtpo=i|\hht=j)$. $\pi\in\RR^m$ denotes
the initial state distribution with $\pi_i = \PP(\hhone=i)$. The emission
densities are $\Obsj:\Xcal\mapsto \RR_+$ for all $j\in [m]$ where
$\Obsj(s) = p(\xt = s|\hht = j)$.

In order to follow~\citet{hsu09hmm}, we need to be able to perform standard
algebraic operations, such as matrix-matrix multiplication or SVD, on the
introduced quantities. Having continuous emission probabilities complicates the
matters and necessitates techniques from continuous linear algebra.

\subsection{A Brief Review of Continuous Linear Algebra}
In this section we introduce continuous analogues of matrices and their
factorisations. We only briefly review those needed for this exposition. For
more details refer to Chapters 3 and 4 of~\citet{townsend14computing}.

A \emph{matrix} $F\in\RR^{m\times n}$ is an $m\times n$ array of numbers where
$F(i,j)$ denotes the entry in row $i$, column $j$. We will also look at cases
where either $m$ or $n$ is infinite. A \emph{column qmatrix} (quasi-matrix)
$Q\in\RR^{[a,b]\times m}$ is a collection of $m$ functions defined on $[a,b]$
where the row index is continuous and column index is discrete. Writing $Q =
[q_1,\dots, q_m]$ where $q_j:[a,b]\mapsto \RR$ is the $j$\ssth function,
$Q(y,j) = q_j(y)$ denotes the  value of the $j$\ssth function at $y\in[a,b]$.
$Q^\top\in\RR^{m\times [a,b]}$ denotes a row qmatrix with $Q^\top(j,y) =
Q(y,j)$. A \emph{cmatrix} (continous-matrix) $C\in\RRm{[a,b]}{[c,d]}$ is a two
dimensional function where both the row and column indices are continuous and
$C(y,x)$ is value of the function at $(y,x) \in [a,b]\times[c,d]$. $C^\top \in
\RRm{[c,d]}{[a,b]}$ denotes its transpose with $C^\top(x,y) = C(y,x)$.

Qmatrices and cmatrices permit all matrix multiplications with suitably
defined inner products. Let
$F \in \RRm{m}{n}$, $Q \in \RRm{[a,b]}{m}$, $P\in \RRm{[a,b]}{n}$,
$R\in \RRm{[c,d]}{m}$ and $C\in\RRm{[a,b]}{[c,d]}$. It follows that
$F(:,j)\in \RRv{m}$, $Q(y,:)\in\RRm{1}{m}$, $Q(:,i)\in\RRv{[a,b]}$,
$C(y,:)\in\RRm{1}{[c,d]}$ etc.
Then the following hold:
\vspace{-0.02in}
\begin{itemize}
\item
\vspace{-0.05in}
$QF = S \in \RRm{[a,b]}{n}\quad$ where
$\quad S(y,j) = Q(y,:) F(:,j) = \sum_{k=1}^m  Q(y,k)F(i,k)$.
\item
\vspace{-0.05in}
$Q^\top P = H\in \RRm{m}{n}\quad$ where
$\quad H(i,j) = Q(:,j)^\top P(:,j) =  \int_a^b Q^\top(i,s)P(s,j)\ud s$.
\item
\vspace{-0.05in}
$QR^\top = D\in \RRm{[a,b]}{[c,d]}\quad$ where
$\quad D(y,x) = Q(y,:)R(x,:)^\top =\sum_{1}^m Q(y,k)R^\top(k,x)$.
% \vspace{-0.05in}
\item
\vspace{-0.05in}
$CR = T\in\RRm{[a,b]}{m}\quad$ where
$\quad T(y,j) = C(y,:)R(:,j) = \int_c^d C(y,s)R(s,j)\ud s$.
\vspace{-0.05in}
\end{itemize}
\vspace{-0.02in}
A cmatrix has a singular value decomposition (SVD).
If $C\in\RRm{[a,b]}{[c,d]}$, an SVD of $C$ is the sum
$
C(y,x) %= U\Sigma V^\top
= \sum_{j=1}^\infty \sigma_j u_j(y)v_j(x),
$
which converges in $\Ltwo$.
% \[
% C(y,x) %= U\Sigma V^\top
% = \sum_{j=1}^\infty \sigma_j u_j(y)v_j(x),
% \]
Here $\sigma_1\geq \sigma_2\geq \dots$.
are the singular values of $C$.
% $\{u_j\}_{j\geq 1}$ are the left singular vectors and $\{v_j\}_{j\geq 1}$ are the right
% singular vectors.  $\{u_j\}_{j\geq 1}, \{v_j\}_{j\geq 1}$ are orthonormal
% % bases for functions on $[a,b]$ and $[c,d]$ respectively, i.e.
% bases $\Ltwo([a,b])$ and $\Ltwo([c,d])$ respectively, i.e.
% $\int_a^b u_j(s)u_k(s)\ud s = \indfone(j=k)$.
$\{u_j\}_{j\geq 1}$ and $\{v_j\}_{j\geq 1}$ are the left and right
singular vectors and form  orthonormal
bases for $\Ltwo([a,b])$ and $\Ltwo([c,d])$ respectively, i.e.
$\int_a^b u_j(s)u_k(s)\ud s = \indfone(j=k)$.
It is known that the SVD of a cmatrix exists uniquely with $\sigma_j \rightarrow 0$,
 and continuous singular vectors
(Theorem 3.2,~\citep{townsend14computing}).
Further, if $C$ is Lipshcitz continuous w.r.t both
variables then
$\sum\sigma^2_j < \infty$ and
the SVD is absolutely and uniformly convergent.
Writing the singular vectors as infinite qmatrices
$U = [u_1, u_2\dots ], V=[v_1,v_2\dots]$,
and $\Sigma = \diag(\sigma_1,\sigma_2\dots )$ we can write the SVD as,
\[
C = U\Sigma V^\top = \sum_{j=1}^\infty \sigma_j U(:,j)V(:,j)^\top.
\]
If only $m<\infty$ singular values are nonzero then we say that $C$ is of rank $m$.
% TODO: Figure ... illustrates a cmatrix SVD.
The SVD of a Qmatrix $Q\in\RRm{[a,b]}{m}$ is,
$
Q = U\Sigma V^\top = \sum_{j=1}^m \sigma_j U(:,j)V(:,j)^\top,
$
where $U\in \RRm{[a,b]}{m}$ and $V\in\RRm{m}{m}$ have orthonormal columns
and $\Sigma = \diag(\sigma_1,\dots,\sigma_m)$ with
$\sigma_1\geq \sigma_2\geq \dots \geq \sigma_m \geq 0$.
The SVD of a qmatrix also exists uniquely (Theorem 4.1,~\citep{townsend14computing}).
The rank of a column qmatrix is the number of linearly independent columns
(i.e. functions) and is equal to the number of nonzero singular values.

Finally, the pseudo inverse of the cmatrix $C$ is $C^\dagger = V \Sigma^{-1}U^\top$ with
$\Sigma^{-1} = \diag( 1/\sigma_1, 1/\sigma_2, \dots )$.
The $p$-operator norm of a cmatrix, for $1\leq p \leq \infty$ is
$\|C\|_p = \sup_{\|x\|_p = 1} \|Cx\|_p$ where
$x\in \RRv{[c,d]}$, $Cx \in \RRv{[a,b]}$, $\|x\|^p_p = \int_c^d (x(s))^p\ud s$ for
$p< \infty$ and $\|x\|_\infty = \sup_{s\in[c,d]} x(s)$.
The Frobenius norm of a cmatrix is $\|C\|_F = \left( \int_a^b\int_c^d C(y,x)^2 \ud x
\ud y \right)^{1/2}$.
It can be shown that $\|C\|_2 = \sigma_1$ and $\|C\|^2_F = \sum_j \sigma_j^2$ where
$\sigma_1\geq \sigma_2 \geq \dots$ are its singular values.
Note that analogous relationships hold with finite matrices.
The pseudo inverse and norms of a qmatrix are similarly defined and similar
relationships hold with its singular values.

% In what follows we will use $\one_{[a,b]}, \zero_{[a,b]}$ to denote functions on
% $[a,b]$ which take values $1$ and $0$ everywhere and $\one_m,\zero_m$ to denote
% $m$-vectors of $1$'s and $0$'s.
\textbf{Additional notation.}
In what follows we will use $\one_{[a,b]}$ to denote the function
taking value $1$ everywhere in $[a,b]$ and $\one_m$ to denote
$m$-vectors of $1$'s.
% When evident from context, we will drop the subscripts.
When we are dealing with $L^p$ norms of a function we will explicitly use the
subscript $L^p$ to avoid confusion with the operator/Frobenius norms of qmatrices and
cmatrices.
For example, for a cmatrix $\|C\|^2_{\Ltwo} = \int\int C(\cdot,\cdot)^2 = \|C\|^2_F$.
As we have already done,
throughout the paper we will overload notation for inner products, multiplications
and pseudo-inverses depending on whether they hold for matrices, qmatrices or
cmatrices.
E.g. when $p,q\in \RR^m, p^\top q  = \sum_1^m p_i q_i$ and when $p,q\in \RR^{[a,b]}$,
$p^\top q = \int_a^b p(s)q(s)\ud s$.
$\PP$ will be used to denote probabilities of events while $p$ will denote
probability density functions (pdf).

\toworkon{\textbf{Q:} It feels like this review is too dense and takes too much space. Which parts of it is better keep and which is better to put into the appendix?}

\subsection{Observable Representation}

% Denoting them as a qmatrix $\Obs =
% [\Obsjj{1},\dots, \Obsjj{m}] \in \RR^{[0,1]\times m}$ we have $\Obs(y,j)
% =\Obsj(y) \geq 0, \forall y\in[0,1], j\in[m]$ and $\onezo^\top \Obs = \onem$.

% In addition, let $\Obsdiag(x) = \diag( \Obsjj{1}(x), \dots, \Obsjj{m}(x))$, and
% $A(x) = T\Obsdiag(x)$. Let $\xotot = \{\xone, \dots, \xt\}$ be an ordered
% sequence and $\xttoo = \{\xt, \dots, \xtt{1}\}$ denote its reverse. For
% brevity, we will overload notation for $A$ for sequences and write $A(\xttoo) =
% A(\xt)A(\xtt{t-1}) \dots A(\xtt{1})$. Then, the joint probability of the
% sequence $\xotot$ can be computed via $p(\xotot) = \onem^\top A(\xttoo)
% \pi$,~\citep{jaeger00observable}.

The observable representation~\citep{jaeger00observable} is a description of a
HMM in terms of quantities that depend on the observations. This representation
is useful for two reasons: (i) as it depends only on the observations they can
be directly estimated from data; (ii) they can be used to compute joint and
conditional probabilities of sequences even without knowledge of $T$ and $\Obs$
and therefore can be used for inference and prediction. First define the joint
probabilities $\Po, \Pto, \Ptto$,
\begin{align*}
\Po(t) = p(\xone=t), \hspace{0.2in}
\Pto(s,t) = p(\xtwo=s, \xone=t) , \hspace{0.2in}
\Ptto(r,s,t) = p(\xthree=r,\xtwo=s,\xone=t).
\end{align*} In addition let, $\Ptxo(r,t) = \Ptto(r, x, t)$ for all
$x\in[0,1]$. We will find it useful to view both $\Pto, \Ptxo \in
\RRm{[0,1]}{[0,1]}$ as cmatrices. In addition to the above, we will also need
an additional qmatrix $U\in \RRm{[0,1]}{m}$ such that $U^\top \Obs \in
\RRm{m}{m}$ is invertible. Given one such $U$, the observable representation of
an HMM is given by the three parameters $\bone, \binf\in \RR^m$ and
$B:[0,1]\mapsto \RRm{m}{m}$,
\begin{align*}
\bone = U^\top \Po, \hspace{0.5in}
\binf = (\Pto^\top U)^\dagger \Po,
\hspace{0.5in} B(x) = (U^\top \Ptxo)(U^\top \Pto)^\dagger
\numberthis \label{eqn:obsRepr}
\end{align*} As before, for a sequence  $\xttoo = \{\xt, \dots, \xtt{1}\}$, we
define $B(\xttoo) = B(\xt)B(\xtt{t-1}) \dots B(\xtt{1})$. The following lemma
shows that the first $m$ left singular vectors of $\Pto$ are a natural choice
for $U$.
\insertprespacing
\begin{lemma} Let $\pi > 0$, $T$ and $\Obs$ be of rank $m$ and $U$ be the
qmatrix composed of the first $m$ left singular vectors of $\Pto$. Then $U^\top
\Obs$ is invertible.
\label{lem:UPtO}
\end{lemma}
% \insertpostspacing
To compute the joint/conditional probabilities using the observable representation,
we will maintain an ``internal state" $\bt$ which will be updated as we see more
observations.
The internal state at time $t$ is
$\bt = B(\xtt{t-1:1}) \bone/ (\binf^\top B(\xtt{t-1:1})\bone)$.
Note that the definition of $\bt$ is consistent with $\bone$.
The following lemma establishes the relationship between the observable
representation $\bone,\binf,B$ and the internal states $\bt$ to the HMM parameters
and probabilities.
\insertprespacing
\begin{lemma}[Properties of the Observable Representation]
Let $\rank(T) = \rank(\Obs) = m$ and $U^\top \Obs$ be invertible.
Let $p(\xotot)$ denote the joint probability of a sequence $\xotot$ and
$p(\xtt{t+1:t+t'}|\xotot)$ denote the conditional proabability of
$\xtt{t+1:t+t'}$ given $\xotot$ in a sequence $\xtt{1:t+t'}$.
Then the following are true.
\vspace{-0.15in}
\begin{enumerate}[itemsep=-1mm]
\item $\bone = \UtO \pi$
\item $\binf = \onem^\top \UtOinv$
\item $B(x) = (\UtO)A(x)\UtOinv$ for all $x\in[0,1]$.
\item $\btpo = B(\xt)\bt / (\binf^\top B(\xt) \bt)$.
% \item $p(\xotot) = \onem^\top A(\xotot) \pi = \binf^\top B(\xotot) \bone$.
\item $p(\xotot)  = \binf^\top B(x_{t:1}) \bone$.
\item $p(\xtt{t+t':t+1}|\xotot) =  \binf^\top B(\xtt{t+t':t+1}) \bt$.
\vspace{-0.02in}
\end{enumerate}
\label{lem:obsProperties}
\end{lemma}
The last two claims of the above lemma show that we can use the observable
representation for computing the joint and conditional probabilities of sequences.
The proofs of Lemmas~\ref{lem:UPtO} and~\ref{lem:obsProperties} is similar to the
discrete case and mimics Lemmas 2, 3 \& 4 of~\citet{hsu09hmm}.

% \begin{proof}[\bf Proof of Lemmas~\ref{lem:UPtO},~\ref{lem:obsProperties}]
% % The proof is similar to the discrete case and mimics the steps in Lemmas 2,3 \& 4
% % of~\citet{hsu09hmm}.
% The proof is similar to the discrete case and mimics Lemmas 2,3 \& 4
% of~\citet{hsu09hmm}.
% % The proof mimics the steps in Lemmas 2,3 \& 4
% % of~\citet{hsu09hmm} for the discrete case.
% \end{proof}

\toworkon{\textbf{Q:} Is this section too dense?}

